ESFL: Efficient Split Federated Learning over Resource-Constrained Heterogeneous Wireless Devices

Federated learning (FL) allows multiple parties (distributed devices) to train a machine learning model without sharing raw data. How to effectively and efficiently utilize the resources on devices and the central server is a highly interesting yet challenging problem. In this paper, we propose an efficient split federated learning algorithm (ESFL) to take full advantage of the powerful computing capabilities at a central server under a split federated learning framework with heterogeneous end devices (EDs). By splitting the model into different submodels between the server and EDs, our approach jointly optimizes user-side workload and server-side computing resource allocation by considering users' heterogeneity. We formulate the whole optimization problem as a mixed-integer non-linear program, which is an NP-hard problem, and develop an iterative approach to obtain an approximate solution efficiently. Extensive simulations have been conducted to validate the significantly increased efficiency of our ESFL approach compared with standard federated learning, split learning, and splitfed learning.

==> sections/DistributedML.tex <==
\section{Distributed Machine Learning}
\label{sec:DistributedML}
In this section, we briefly discuss two distributed machine learning schemes, namely, federated learning and split learning, to facilitate the introduction of our ESFL, as our ESFL is based on these two schemes. 

\subsection{Federated Learning~\cite{mcmahan2017communication}}
Considering $S$ different datasets $\left\{ \mathcal{D}_{1}, ..., \mathcal{D}_{S} \right\}$ held by $S$ users or EDs, and all of them agree to train an ML model by leveraging their respective datasets. User $i$ collects a data matrix $\mathcal{D}_{i} = \{X_i, Y_i\}$, consisting of an input data matrix $X_i = [x_{i, 1}, ..., x_{i, n_i}]$ and an output label vector $Y_i = [y_{i, 1}, ..., y_{i, n_i}]$, where $n_i$ is the number of data samples held by user $i$. To train an ML model, we attempt to minimize loss function $\mathcal{l}(x_{i, k}, \hat{y}_{i, k},y_{i, k}; \mathcal{w})$, where $\hat{y}_{i, k}$ is the predicted result generated by the input data $x_{i, k}$ given the model parameters $\mathcal{w}$. To simplify the notation, we use $f_{i, k}(\mathcal{w})$ to represent the loss function $\mathcal{l}(x_{i, k}, \hat{y}_{i, k},y_{i, k}; \mathcal{w})$ in which
\begin{equation}
    \begin{gathered}
        \min_{\mathcal{w}} f_i(\mathcal{w}) = \frac{1}{n_i}\sum_{k = 1}^{n_i} f_{i, k}(\mathcal{w}).
    \end{gathered}
\end{equation}
The coordinating server aggregates the uploaded local ML model updates and obtains the $r$-th round global ML model by minimizing the global loss function $F(\mathcal{w}_r)$. The objective function of the global ML model is
\begin{equation}
    \begin{gathered}
        \min_{\mathcal{w}} F(\mathcal{w}_r) = \frac{1}{N}\sum_{i = 1}^{S} n_if_{i}(\mathcal{w}),
    \end{gathered}
\end{equation}
where $N = \sum_{i = 1}^{S} n_i$ is the total number of training samples.

\subsection{Split Learning~\cite{poirot2019split}}
Similar to federated learning, we consider there are $M$ users and one central server participating split learning. Since the key idea of split learning (SL) is to split the whole training procedure into multiple parts and deploy them between users and the server, the whole ML model is split into the user-side model $M^c_i$ and the server-side model $M^s$, where user $i$ holds a local dataset $\mathcal{D}_{i}$ and a local user-side model $M^c_i$, and the server holds one server-side model $M^s$ that is updated by all users. The entire training procedure consists of $R$ rounds of $T$ iterations. 

More specifically, in the $k$-th iteration, the user-side model $M^c_i$ and server-side model $M^s$ are updated in the following few steps\cite{vepakomma2018no}:

\begin{itemize}
    \item [\textbf{1)}] A mini-batch $(x_{i, k}, y_{i, k})$ sampled from dataset $\mathcal{D}_{i}$ is passed through the user-side model $M^c_i$ to produce activation $A_{i, k} = M^c_i(x_{i, k})$, where we refer to $A_{i, k}$ as the \textit{split activation} generated by user $i$.
    \item [\textbf{2)}] User $i$ sends the data-label pair $(A_{i, k}, y_{i, k})$ to the server.
    \item [\textbf{3)}] The server generates predicted result $\hat{y}_{i, k} = M^s(A_{i, k})$ and computes the loss function $\nabla L(\hat{y}_{i, k}, y_{i, k})$ to update the server-side model $M^s$.
    \item [\textbf{4)}] The server employs the backpropagation to compute the \textit{updated split activation} $\hat{A}_{i, k}$ and sends back to user $i$.
    \item [\textbf{5)}] User $i$ computes the difference $\nabla A_{i, k}$ based on $A_{i, k}$ and $\hat{A}_{i, k}$ to update the user-side model $M^c_i$.  
\end{itemize}

